3D Packing for Self-Supervised Monocular Depth Estimation

Although cameras are ubiquitous, robotic platforms typically rely on active sensors like LiDAR for direct 3D perception. In this work, we propose a novel self-supervised monocular depth estimation method combining geometry with a new deep network, PackNet, learned only from unlabeled monocular videos. Our architecture leverages novel symmetrical packing and unpacking blocks to jointly learn to compress and decompress detail-preserving representations using 3D convolutions. Although self-supervised, our method outperforms other self, semi, and fully supervised methods on the KITTI benchmark. The 3D inductive bias in PackNet enables it to scale with input resolution and number of parameters without overfitting, generalizing better on out-of-domain data such as the NuScenes dataset. Furthermore, it does not require large-scale supervised pretraining on ImageNet and can run in real-time. Finally, we release DDAD (Dense Depth for Automated Driving), a new urban driving dataset with more challenging and accurate depth evaluation, thanks to longer-range and denser ground-truth depth generated from high-density LiDARs mounted on a fleet of self-driving cars operating world-wide.

==> latex/results/ATE-accuracy.tex <==
\begin{table*}
\centering
{
\small
\setlength{\tabcolsep}{1.0em}
\begin{tabular}{lccccc}
\toprule
\textbf{Method} &
Supervision & 
Resolution & 
GT & 
\quad Seq. 09\quad & 
\quad Seq. 10\quad \\
\midrule
Godard et al.~\cite{godard2018digging}                           & M    & 640 x 192 & \checkmark & 0.023 $\pm$ 0.013 & 0.018 $\pm$ 0.014 \\
SfMLearner (Zhou et al.~\cite{zhou2017unsupervised})             & M    & 416 x 128 & \checkmark & 0.021 $\pm$ 0.017 & 0.020 $\pm$ 0.015 \\
DF-Net~\cite{zou2018dfnet}                                       & M    & 576 x 160 & \checkmark & 0.017 $\pm$ 0.007 & 0.015 $\pm$ 0.009 \\
Klodt et al.~\cite{klodt2018supervising}                         & M    & 416 x 128 & \checkmark & 0.014 $\pm$ 0.007 & 0.013 $\pm$ 0.009 \\
Vid2Depth~\cite{mahjourian2018unsupervised}                      & M    & 416 x 128 & \checkmark & 0.013 $\pm$ 0.010 & 0.012 $\pm$ 0.011 \\
GeoNet (Yin et al.~\cite{yin2018geonet})                         & M    & 416 x 128 & \checkmark & 0.012 $\pm$ 0.007 & 0.012 $\pm$ 0.009 \\
Struct2Depth~\cite{casser2018depth}                              & M    & 416 x 128 & \checkmark & 0.011 $\pm$ 0.006 & 0.011 $\pm$ 0.010 \\
\midrule
\textbf{PackNet-SfM}                                             & M    & 640 x 192 & \checkmark & 0.009 $\pm$ 0.005 & 0.008 $\pm$ 0.007 \\
\textbf{PackNet-SfM}                                             & M+v  & 640 x 192 & \checkmark & 0.008 $\pm$ 0.005 & 0.008 $\pm$ 0.007 \\
\textbf{PackNet-SfM}                                             & M+v  & 640 x 192 &            & 0.012 $\pm$ 0.006  & 0.011 $\pm$ 0.007 \\
\bottomrule
\end{tabular}\\\vspace{1mm}
}
\caption{\textbf{Average Absolute Trajectory Error (ATE) in meters on the KITTI Odometry Benchmark~\cite{geiger2013vision}}: All methods are trained on Sequences 00-08 and evaluated on Sequences 09-10. The ATE numbers are averaged over all overlapping 5-frame snippets in the test sequences. \text{M+v} refers to velocity supervision (v) in addition to monocular images (M). The \textit{GT} checkmark indicates the use of ground-truth translation to scale the estimates at test-time.}
\label{table:supplementary-pose-ate}
\end{table*}



==> latex/results/depth-accuracy-backbones.tex <==
\begin{table*}
\centering
\small
{
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{lccccccccccc}
\toprule
\textbf{Backbone} &
Pretrained & 
Abs Rel &
Sq Rel &
RMSE &
RMSE log &
$\delta<1.25$ &
$\delta<1.25^2$ &
$\delta<1.25^3$\vspace{0.5mm}\\
\midrule
ResNet18  & & 0.145 & 1.457 & 5.842 & 0.226 & 0.820 & 0.937 & 0.973  \\
ResNet18  & \cmark & 0.142 & 1.352 & 5.969 & 0.223 & 0.823 & 0.940 & 0.974  \\
\midrule
ResNet34  & & 0.140 & 1.547 & 5.979 & 0.222 & 0.832 & 0.941 & 0.974  \\
ResNet34  & \cmark & 0.141 & 1.359 & 5.605 & 0.219 & 0.834 & 0.943 & 0.974  \\
\midrule
ResNet50  & & 0.141 & 1.208 & 5.668 & 0.221 & 0.828 & 0.939 & 0.974  \\
ResNet50  & \cmark & 0.138 & 1.253 & 5.606 & 0.217 & 0.833 & 0.943 & 0.976  \\
\midrule
ResNet101  & & 0.139 & 1.199 & 5.614 & 0.220 & 0.829 & 0.941 & 0.975  \\
ResNet101  & \cmark & 0.140 & 1.397 & 5.901 & 0.219 & 0.833 & 0.944 & 0.975  \\
\midrule
\textbf{PackNet} & & \textbf{0.120} & \textbf{1.018} & \textbf{5.136} & \textbf{0.198} & \textbf{0.865} & \textbf{0.955} & \textbf{0.980}\\
\hline
\bottomrule
\end{tabular}
}\vspace{1mm}
\caption{\textbf{\textit{ResNet} Backbone comparisons}. For the various ResNet backbones, we report monocular depth estimation results on the KITTI dataset~\cite{geiger2013vision} using the Eigen Split~\cite{eigen2014depth}, and how they compare to \textit{PackNet} under the same training conditions. For completeness, we provide results for both training from random initialization and with \textit{ImageNet} \cite{Deng09imagenet} pre-training.}
\label{table:depth-accuracy-backbones}
\end{table*}

==> latex/results/improved_gt.tex <==

\begin{table*}[t!]
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{lccccccccccccc}
\toprule
\textbf{Method} &
Supervision & 
Resolution & 
Dataset &
Abs Rel &
Sq Rel &
RMSE &
RMSE$_{log}$ &
$\delta < 1.25$ &
$\delta < 1.25^2$ &
$\delta < 1.25^3$\vspace{0.5mm}\\
\toprule
SfMLeaner~\cite{zhou2017unsupervised} & M & 416 x 128 & K & 
0.176 & 1.532 & 6.129 & 0.244 & 0.758 & 0.921 & 0.971\\
Vid2Depth~\cite{mahjourian2018unsupervised} & M & 416 x 128 & K & 
0.134 & 0.983 & 5.501 & 0.203 & 0.827 & 0.944 & 0.981\\
GeoNet~\cite{yin2018geonet} & M & 416 x 128 & K & 
0.132 & 0.994 & 5.240 & 0.193 & 0.8833 & 0.953 & 0.985\\
DDVO~\cite{wang2018learning} & M & 416 x 128 & K & 
0.126 & 0.866 & 4.932 & 0.185 & 0.851 & 0.958 & 0.986\\
Ranjan~\cite{advcollab} & M & 640 x 192 & K & 
0.123 & 0.881 & 4.834 & 0.181 & 0.860 & 0.959 & 0.985\\
EPC++~\cite{epc++} & M & 640 x 192 & K & 
0.120 & 0.789 & 4.755 & 0.177 & 0.856 & 0.961 & 0.987\\
Monodepth2$^\ddagger$ ~\cite{godard2017unsupervised} & M & 640 x 192 & K & 
0.090 & 0.545 & 3.942 & 0.137 & 0.914 & 0.983 & 0.995\\
\midrule
DORN$^\ddagger$ & Sup. & 513 x 385 & K & 
\textbf{0.072} & \textbf{0.307} & \textbf{2.727} & 0.120 & 0.932 & 0.984 & 0.995\\
\midrule
%WITH_PP_GT | Avg abs_rel :   0.078, sq_rel :   0.420, rmse :   3.485, rmse_log :   0.121, a1 :   0.931, a2 :   0.986, a3 :   0.996
\textbf{PackNet-SfM} & M & 640 x 192 & K & 
0.078 & 0.420 & 3.485 & 0.121 & 0.931 & 0.986 & 0.996\\
%WITH_PP_GT | Avg abs_rel :   0.072, sq_rel :   0.359, rmse :   3.153, rmse_log :   0.109, a1 :   0.945, a2 :   0.991, a3 :   0.997
\textbf{PackNet-SfM} & M & 1280 x 384 & CS + K & 
\textbf{0.072} & 0.359 & 3.153 & \textbf{0.109} & \textbf{0.945} & \textbf{0.991} & \textbf{0.997}\\
\bottomrule
\end{tabular}
}
\caption{\textbf{Quantitative performance comparison of PackNet-SfM on the KITTI dataset}
(improved ground-truth depth maps~\cite{gtkitti}, for reported depths of up to 80m)}.
\label{table:improved-gt}
\end{table*}

==> latex/results/kitti_eigen_traj_results.tex <==

\begin{table*}[!t]
\centering
\tiny
\setlength{\tabcolsep}{.7em}
\begin{tabular}{lcccccccccccccc}

\textbf{Method} & \textbf{Sensor} & 01$^*$ &    02$^*$  &  06$^*$  &  08$^*$   &   09$^*$  & 10$^*$   & 00$^\dagger$  & 03$^\dagger$  & 04$^\dagger$  & 05$^\dagger$  & 07$^\dagger$  & \textbf{Train Avg} & \textbf{Test Avg} \\
\toprule

& \multicolumn{12}{c}{$t_{rel}$ - Average Translational RMSE drift (\%) on trajectories of length 100-800m.}  \\
\midrule
SuperDepth~\cite{pillai2018superdepth}           & Stereo & 13.48 & 3.48 & 1.81  & 2.25  &  3.74 &  2.26 & 6.12  & 7.90  & 11.80 &  4.58 & 7.60  & 4.50  & 7.60  \\
DeepVO~\cite{wang2017deepvo}                    &Mono+Pose&   -   &   -   & 5.42 &   -   &   -   &8.11   &   -   & 8.49 &  7.19 &  2.62 &  3.91  &   -   & 5.96  \\
% Zhu et al~\cite{zhu2018robustness}               & Mono+RANSAC & 45.5  &  6.40 &  3.49 &   4.08 & 4.66 & 6.30 &  4.95 & 4.83  & 2.43 &  3.97 &  4.50 & 8.91  & 5.48  \\
Velas et al.~\cite{velas2018cnn}                &Lidar+IMU& 4.44  & 3.42 & 1.88  & 2.89  &  4.94 & 3.27  & 3.02  & 4.94  & 1.77  &  2.35 & 1.77  &  3.11 & 3.22  \\ 
VISO2\_S~\cite{geiger2011stereoscan}             & Stereo &   -   &   -   & 1.48 &   -   &   -   &  1.17 &  -    & 3.21  & 2.12  &  1.53 &  1.85 &  -    & 1.89  \\
LO-NET~\cite{li2019net}                          & Lidar  &  1.36 & 1.52  & \textbf{0.71} &  2.12 &  1.37 &  1.80 & 1.47  & 1.03  &  0.51 &  1.04 &  1.70 & 1.09  & 1.75  \\
LOAM~\cite{zhang2017low}                         & Lidar  &  \textbf{0.78} &  1.43 & 0.92 &  \textbf{0.86} &  \textbf{0.71} &  \textbf{0.57} & \textbf{0.65}  &  \textbf{0.63} &  1.12 &  0.77 &  0.79 &  -    &  1.33  \\ 
ORB-SLAM2~\cite{mur2017orb}                      & Stereo  &  1.38 &  \textbf{0.81} & 0.82 &  1.07 &  0.82 &  0.58 & 0.83  &  0.71 &  0.45 &  0.64 &  0.78 &  -    & 0.81  \\
DVSO~\cite{yang2018deep}                         & Stereo &  1.18 &  0.84 & \textbf{0.71} &  1.03 &  0.83 &  0.74 & 0.71  &  0.77 &  \textbf{0.35} &  \textbf{0.58} &  \textbf{0.73} & \textbf{0.89}  & \textbf{0.63}  \\
\midrule
% \href{https://app.wandb.ai/tri/monodepth-test/runs/yszqdqy6/overview}
CoRL Pose (snippet scale)                       & Mono   & 17.59 &  6.82 & 8.93 &  8.38 &  6.49 & 9.83 &  7.16 &  7.66 & 3.8   &   6.6 &  11.48 & 9.67 &  7.34 \\
CoRL Pose (Sim3)                                & Mono   &  4.74 &  2.6  & 0.97 &  1.72 & 1.98 &  2.56 & 3.83 &   5.74 &  1.45 &  1.54 &  2.94 &  2.43 &  3.1  \\
Our F2F (snippet scale)                    & Mono   & - & - & - &  - &  - & - &  7.16 &  7.66 & 3.8   &   6.6 &  - & - &  2.05 \\
Our F2F (Sim3)                             & Mono   & - & - & - &  - &  - & - & 3.83 &   5.74 &  1.45 &  1.54 &  - &  - &  3.1411  \\
Our DS-DSO (Sim3)                             & Mono   & - & - & - &  - &  - & - & 2.184 &  2.095 &   1.196 &  2.370 &  1.764 &  - &  1.922  \\
\midrule
& \multicolumn{12}{c}{$r_{rel}$ - Average Rotational RMSE drift ($^{{\circ}}/100m$) on trajectories of length 100-800m.} \\ 
\midrule
SuperDepth~\cite{pillai2018superdepth}           & Stereo & 1.97 & 1.10 & 0.78 & 0.84 & 1.19 & 1.03 & 2.72& 4.30  & 1.90 & 1.67 & 5.17 & 1.15 & 3.15 \\
DeepVO~\cite{wang2017deepvo}                    &Mono+Pose&   -  &  -   & 5.82 &   -  &   -  & 8.83 &  -   & 6.89 & 6.97 & 3.61 & 4.60 &  -  & 6.12 \\
% Zhu et al~\cite{zhu2018robustness}               & Mono+RANSAC & 1.78 & 1.92 & 1.02 & 1.17 & 1.69  & 
VISO2\_S~\cite{geiger2011stereoscan}             & Stereo &   -  &   -  & 1.58 & -    &   -  & 1.30 & -    & 3.25 & 2.12 & 1.60 & 1.91 &  -   &  1.96\\
LO-NET~\cite{li2019net}                          & Lidar  & 0.47 & 0.71 & 0.50 & 0.77 & 0.58 & 0.93 & 0.72 & 0.66 & 0.65 & 0.69 & 0.89 &  0.63& 0.79 \\
ORB-SLAM2~\cite{mur2017orb}                      & Stereo & 0.20 & 0.28 & 0.25 & 0.31 & 0.25 & 0.28 & 0.29 & 0.17 & 0.18 & 0.26 & 0.42 & -   & 0.26 \\
DVSO~\cite{yang2018deep}                         & Stereo & \textbf{0.11} & \textbf{0.22} & \textbf{0.20} &
\textbf{0.25} & \textbf{0.21} & \textbf{0.21} & \textbf{0.24} & \textbf{0.18} & \textbf{0.06} & \textbf{0.22} & \textbf{0.35} & \textbf{0.20} & \textbf{0.21} \\
\midrule
CoRL Pose                                     & Mono   & 1.01 & 0.87 & 0.39 & 0.61 & 0.86 & 0.98 & 1.70 & 3.49 & 0.42 & 0.90 & 2.05 & 0.79 & 1.71\\

Our DS-DSO (Sim3)                             & Mono   & - & - & - &  - &  - & - & 0.4268 & 0.2782 & 0.2255 &  0.3217 & 0.6342 &  - &  0.3773  \\
\bottomrule
\end{tabular}

\caption{Comparison to direct, feature based, lidar based and other learned methods on the KITTI odometry benchmark. We report the following metrics $t_{rel}$ and $r_{rel}$ averaged over trajectories of length 100-800m. $\dagger$ and $*$ represent test and respectively train seq. for our method, as well as for~\cite{pillai2018superdepth, yang2018deep}. \cite{li2019net} and~\cite{velas2018cnn} are trained on Seq. 00-06 and tested on Seq. 07-10. DeepVO~\cite{wang2017deepvo} is trained on Seq. 00, 02, 08 and 09. The numbers for~\cite{velas2018cnn} are taken from~\cite{li2019net}. The results of the methods trained only with Mono data were scaled using ground truth depth scale.}
\label{table:kitti-eigen-traj} 
\vspace{-5mm}
\end{table*}




% ds-dsoboom -- Mean TRAJ (pos: 2.1840, rot: 0.4268)

% ds-dsoboom -- Mean TRAJ (pos: 2.0958, rot: 0.2782)

% ds-dsoboom -- Mean TRAJ (pos: 1.1967, rot: 0.2255)

% ds-dsoboom -- Mean TRAJ (pos: 2.3709, rot: 0.3217)

% ds-dsoboom -- Mean TRAJ (pos: 1.7646, rot: 0.6342)

% ds-dsoboom -- Overall Mean TRAJ (pos: 1.9224, rot: 0.3773)




==> latex/results/packnet-ablation.tex <==
\begin{table*}[t!]
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{lccccccc}
\toprule
\textbf{Depth Network} & 
Abs Rel &
Sq Rel &
RMSE &
RMSE$_{log}$ &
$\delta<1.25$ &
$\delta<1.25^2$ &
$\delta<1.25^3$\vspace{0.5mm}\\
\midrule
%PackNet-SfM w/o 3D Conv. and SR & & \checkmark & 0.128 & 1.102 & 5.286 & 0.207 & 0.852 & 0.949 & 0.977  
%\\
%PackNet-SfM w/o 3D Conv. & & \checkmark & 0.126 & 0.961 & 5.071 & 0.205 & 0.853 & 0.950 & 0.979
%\\
%PackNet-SfM w/o SR & & \checkmark & 0.125 & 1.074 & 5.137 & 0.204 & 0.855 & 0.951 & 0.979
%\\
%PackNet-SfM & & \checkmark & 0.120 & 1.018 & 5.136 & 0.198 & 0.865 & 0.955 & 0.980\\
%PackNet-SfM & \checkmark & & 0.118 & 0.915 & 5.035 & 0.209 & 0.847 & 0.947 & 0.977 \\
%PackNet-SfM & \checkmark & \checkmark & 0.120 & 0.892 & 4.898 %& 0.196 & 0.864 & 0.954 & 0.980 \\
%\midrule
%WITH_PP_GT | Avg abs_rel :   0.133, sq_rel :   1.023, rmse :   5.123, rmse_log :   0.211, a1 :   0.845, a2 :   0.948, a3 :   0.977 
ResNet18 & 0.133 & 1.023 & 5.123 & 0.211 & 0.845 & 0.948 & 0.977
\\
%WITH_PP_GT | Avg abs_rel :   0.120, sq_rel :   0.896, rmse :   4.869, rmse_log :   0.198, a1 :   0.868, a2 :   0.956, a3 :   0.981 
ResNet18$^\ddagger$ & 0.120 & 0.896 & 4.869 & 0.198 & 0.868 & 0.956 & 0.981
\\
%WITH_PP_GT | Avg abs_rel :   0.127, sq_rel :   0.977, rmse :   5.023, rmse_log :   0.205, a1 :   0.856, a2 :   0.953, a3 :   0.978 
ResNet50 & 0.127 & 0.977 & 5.023 & 0.205 & 0.856 & 0.953 & 0.978
\\
%WITH_PP_GT | Avg abs_rel :   0.117, sq_rel :   0.900, rmse :   4.826, rmse_log :   0.196, a1 :   0.873, a2 :   0.958, a3 :   0.980
ResNet50$^\ddagger$ & 0.117 & 0.900 & 4.826 & 0.196 & 0.873 & 0.958 & 0.980
\\
\midrule
%WITH_PP_GT | Avg abs_rel :   0.118, sq_rel :   0.802, rmse :   4.656, rmse_log :   0.194, a1 :   0.868, a2 :   0.956, a3 :   0.981 
PackNet18 & 0.118 & 0.802 & 4.656 & 0.194 & 0.868 & 0.956 & 0.981
\\
%WITH_PP_GT | Avg abs_rel :   0.114, sq_rel :   0.818, rmse :   4.621, rmse_log :   0.190, a1 :   0.875, a2 :   0.959, a3 :   0.981 
PackNet50 & 0.114 & 0.818 & 4.621 & 0.190 & 0.875 & 0.959 & 0.981 
\\
\midrule
%WITH_PP_GT | Avg abs_rel :   0.122, sq_rel :   0.880, rmse :   4.816, rmse_log :   0.198, a1 :   0.864, a2 :   0.955, a3 :   0.980 
PackNet-SfM \small{(w/o packing/unpacking)} & 0.122 & 0.880 & 4.816 & 0.198 & 0.864 & 0.955 & 0.980 
\\
%WITH_PP_GT | Avg abs_rel :   0.118, sq_rel :   0.922, rmse :   4.831, rmse_log :   0.195, a1 :   0.872, a2 :   0.957, a3 :   0.980 
PackNet-SfM \small{(w/o 3D convolutions)} & 0.118 & 0.922 & 4.831 & 0.195 & 0.872 & 0.957 & 0.980 
\\
%WITH_PP_GT | Avg abs_rel :   0.111, sq_rel :   0.785, rmse :   4.601, rmse_log :   0.189, a1 :   0.878, a2 :   0.960, a3 :   0.982 
\textbf{PackNet-SfM} & \textbf{0.111} & \textbf{0.785} & 4.601 & 0.189 & 0.878 & \textbf{0.960} & \textbf{0.982} \\
%WITH_PP_GT | Avg abs_rel :   0.112, sq_rel :   0.798, rmse :   4.573, rmse_log :   0.188, a1 :   0.879, a2 :   0.960, a3 :   0.982 
%\textbf{PackNet-SfM}$^\ddagger$ & `` & `` & 0.112 & 0.798 & \textbf{4.573} & \textbf{0.186} & \textbf{0.879} & \textbf{0.960} & \textbf{0.982} 
\bottomrule
\end{tabular}
}
\caption{\textbf{Ablation studies on the PackNet architecture}, on the KITTI dataset for 640 x 192 resolution (the same PoseNet architecture was used in all depth network variations). \textit{ResNetXX} indicates the use of that specific Residual Network~\cite{he2016deep} version as the encoder, with and without ImageNet~\cite{Deng09imagenet} pretraining. Similarly, \textit{PackNetXX} indicates the use of the same ResNet encoder architecture, but replacing convolutional striding and pooling operations with packing (Sec. \ref{subsec:packing_block}) and upsampling operations with unpacking (Sec. \ref{subsec:unpacking_block}). Finally, we show results with the proposed \textit{PackNet} architecture, first without packing and unpacking (replaced respectively with convolutional striding and bilinear upsampling); then without 3D convolutions on the packing and unpacking blocks (Fig. \ref{fig:modules}); and finally the full proposed architecture, as described in Table \ref{tab:packnet-arch}. The symbol $^\ddagger$ denotes ImageNet \cite{Deng09imagenet} pretraining.} %Frames per second (FPS) values are calculated using a \textit{Titan V100} graphics card, for a batch size of 1. }
%The same depth decoder and pose network were used in all ablation experiments.}

%\textit{3D Conv.} indicates the addition of a 3D convolutional layer to the packing and unpacking blocks (Section \ref{sec:packnet-architecture}); and
%\textit{SR} indicates the use of super-resolution on the output inverse depth maps (Section \ref{sec:superresolution}). All evaluation is performed on the KITTI dataset at resolution of 640 x 192.}
\label{table:packnet-ablation}
\vspace{-3mm}
\end{table*}


==> latex/results/packnet-ablation2.tex <==
\begin{table}[t!]
\centering
{
\small
\setlength{\tabcolsep}{0.2em}
\begin{tabular}{lccccc}
\toprule
\textbf{Depth Network} & 
Abs Rel &
Sq Rel &
RMSE &
RMSE$_{log}$ &
$\delta<1.25$ \vspace{0.5mm}\\
\midrule
ResNet18 & 0.133 & 1.023 & 5.123 & 0.211 & 0.845 
\\
ResNet18$^\ddagger$ & 0.120 & 0.896 & 4.869 & 0.198 & 0.868 
\\
ResNet50 & 0.127 & 0.977 & 5.023 & 0.205 & 0.856 
\\
ResNet50$^\ddagger$ & 0.117 & 0.900 & 4.826 & 0.196 & 0.873 
\\
\midrule
PackNet18 & 0.118 & 0.802 & 4.656 & 0.194 & 0.868 
\\
PackNet50 & 0.114 & 0.818 & 4.621 & 0.190 & 0.875 
\\
\midrule
PackNet-SfM & \multirow{2}{*}{0.122} & \multirow{2}{*}{0.880} & \multirow{2}{*}{4.816} & \multirow{2}{*}{0.198} & \multirow{2}{*}{0.864} \\
\small{(w/o pack/unpack)} & 
\\
PackNet-SfM & \multirow{2}{*}{0.118} & \multirow{2}{*}{0.922} & \multirow{2}{*}{4.831} & \multirow{2}{*}{0.195} & \multirow{2}{*}{0.872}  \\
\small{(w/o 3D convs.)} & & & & &
\\
\textbf{PackNet-SfM} & \textbf{0.111} & \textbf{0.785} & \textbf{4.601} & \textbf{0.189} & \textbf{0.878}  \\
\bottomrule
\end{tabular}
}
\caption{\textbf{Ablation study on the PackNet architecture}, on the standand KITTI benchmark for 640 x 192 resolution. \textit{ResNetXX} indicates that specific architecture~\cite{he2016deep} as encoder, with and without ImageNet~\cite{Deng09imagenet} pretraining (denoted with $\ddagger$). Similarly, \textit{PackNetXX} indicates the same ResNet encoder architecture, but replacing convolutional striding and pooling operations with packing and upsampling operations with unpacking. Finally, we show results with the proposed \textit{PackNet} architecture, first without packing and unpacking (replaced respectively with convolutional striding and bilinear upsampling); then without 3D convolutions on the packing and unpacking blocks; and finally the full proposed architecture.} %The symbol $^\ddagger$ denotes ImageNet \cite{Deng09imagenet} pretraining.} %Frames per second (FPS) values are calculated using a \textit{Titan V100} graphics card, for a batch size of 1. }
%The same depth decoder and pose network were used in all ablation experiments.}

%\textit{3D Conv.} indicates the addition of a 3D convolutional layer to the packing and unpacking blocks (Section \ref{sec:packnet-architecture}); and
%\textit{SR} indicates the use of super-resolution on the output inverse depth maps (Section \ref{sec:superresolution}). All evaluation is performed on the KITTI dataset at resolution of 640 x 192.}
\label{table:packnet-ablation}
\vspace{-6mm}
\end{table}


==> latex/results/qualitative-packnet.tex <==
\begin{figure}[b!]
\centering
   \centering
   {{\renewcommand{\arraystretch}{0.1}
    \setlength{\tabcolsep}{0.1mm}
    \begin{tabular}{cc}

    \includegraphics[width=0.48\columnwidth]{latex/figures/teaser27.png} & 
    \includegraphics[width=0.48\columnwidth]{latex/graphics/1024x384/packnet_cs03.png} \\
    \includegraphics[width=0.48\columnwidth]{latex/figures/teaser51.png} &     
    \includegraphics[width=0.48\columnwidth]{latex/graphics/1024x384/packnet_cs04.png} \\
    \includegraphics[width=0.48\columnwidth]{latex/figures/teaser305.png} &
    \includegraphics[width=0.48\columnwidth]{latex/graphics/1024x384/packnet_cs05.png}\\

    
%    \includegraphics[width=0.9\columnwidth]{latex/figures/teaser_0000001807.png}& 
%    \includegraphics[width=0.9\columnwidth]{latex/figures/teaser27.png}& 
%    %\includegraphics[width=0.9\columnwidth]{latex/figures/000000051_rgb.jpg}& 
%   \includegraphics[width=0.9\columnwidth]{latex/graphics/1024x384/packnet_cs03.png}\\
   
%    \includegraphics[width=0.9\columnwidth]{latex/figures/teaser_0000002351.png} &
%    \includegraphics[width=0.9\columnwidth]{latex/figures/teaser51.png}&    
%    %\includegraphics[width=0.9\columnwidth]{latex/figures/000000051.jpg}& 
%    \includegraphics[width=0.9\columnwidth]{latex/graphics/1024x384/packnet_cs04.png}\\ 

%    \includegraphics[width=0.9\columnwidth]{latex/figures/teaser_0000001768.png}&
%    \includegraphics[width=0.9\columnwidth]{latex/figures/teaser305.png}&
%    \includegraphics[width=0.9\columnwidth]{latex/graphics/1024x384/packnet_cs05.png}\\

   \end{tabular}}}
    \vspace{1mm}
    \caption{\textbf{High-resolution qualitative results of PackNet on the KITTI (left) and CityScapes (right) datasets.}~We illustrate the fine depth detail and crisp boundaries estimated by our proposed \textit{PackNet-SfM} model on diverse set of scenarios. We show that our model is able to achieve state-of-the-art performance while providing strong generalization capability, which is equally critical for driving related tasks.}
    \label{fig:qualitative-depth-2}
\end{figure}

==> latex/results/velocity-supervision.tex <==
% -------------------------------------------------
% PackNet Module Illustration
\begin{figure}[b]
    \centering
    {
    \small
    \setlength{\tabcolsep}{0.3em}
    \begin{tabular}{cc}
    \includegraphics[width=0.5\columnwidth,trim={0mm 0mm 0mm 0mm},clip]{latex/figures/velocity_supervision_abs_rel_vs_epochs.pdf}&
    \includegraphics[width=0.5\columnwidth,trim={0mm 0mm 0mm 0mm},clip]{latex/figures/velocity_supervision_a1_vs_epochs.pdf}
    \end{tabular}}
    \vspace{-2mm}
    \caption{\textbf{Learning scale-aware depth from velocity supervision}. Illustrated above are plots of the Abs. Rel. and $\delta < 1.25$ depth estimation metrics for a monocular with velocity supervision (M+v) model, after each training epoch. Note that initially an unscaled model is learned (black line), that requires ground-truth (GT) for a proper evaluation. Once it stabilizes, scale-awareness starts to gradually be incorporated (red line) until eventually both ground-truth and velocity scaled estimates reach similar values.}
    \label{fig:velocity-supervision}
\end{figure}






